Price of Anarchy of Simple Auctions with Interdependent Values

We expand the literature on the price of anarchy (PoA) of simultaneous item auctions by considering settings with correlated values; we do this via the fundamental economic model of interdependent values (IDV). It is well-known that in multi-item settings with private values, correlated values can lead to bad PoA, which can be polynomially large in the number of agents $n$. In the more general model of IDV, we show that the PoA can be polynomially large even in single-item settings. On the positive side, we identify a natural condition on information dispersion in the market, termed $\gamma$-heterogeneity, which enables good PoA guarantees. Under this condition, we show that for single-item settings, the PoA of standard mechanisms degrades gracefully with $\gamma$. For settings with $m>1$ items we show a separation between two domains: If $n \geq m$, we devise a new simultaneous item auction with good PoA (with respect to $\gamma$), under limited information asymmetry. To the best of our knowledge, this is the first positive PoA result for correlated values in multi-item settings. The main technical difficulty in establishing this result is that the standard tool for establishing PoA results -- the smoothness framework -- is unsuitable for IDV settings, and so we must introduce new techniques to address the unique challenges imposed by such settings. In the domain of $n \ll m$, we establish impossibility results even for surprisingly simple scenarios.

==> appx-multiple-neg.tex <==
\mainneg*
Before proving the theorem, we provide some useful claims. 
We first establish a lower bound on $\opt$.

\begin{claim} \label{clm:opt-lb}
	$\opt=\Omega(n\ln n/\ln\ln n)$.
\end{claim}

\begin{proof}
	We partition the items into $n$ sets of $n$ items. It suffices to show that in each of the sets, $\E_\s[\max_{\ell\in [n]}v_{i\ell}(\s)]=\Omega(\log n/\log\log n)$, since we can allocate the best items in each set to a different bidder. 
	
	The probability that an item's value is at least $k+1$ is 
	\begin{eqnarray}
	\Pr_{\s}\left[ v_{i\ell}(\s)\geq k+1\right] &= &\Pr_\s\left[\sum_{i\in [n]}s_{i\ell}\geq k\right]\nonumber\\
	&\geq & \Pr_\s\left[\sum_{i\in [n]}s_{i\ell}= k\right]\nonumber\\
	& = & \binom{n}{k}\left(\frac{1}{n}\right)^k\left(1-\frac{1}{n}\right)^k\nonumber\\
	&\geq& \left(\frac{n}{k}\right)^k\frac{1}{n^k}\frac{1}{e}\nonumber\\
	& = &\frac{1}{ek^k}.
	\end{eqnarray}
	
	Setting $k=\frac{\ln n}{3\ln\ln n}$, we have $k^k\leq \ln n^{\frac{\ln n}{3\ln\ln n}}=e^{\frac{\ln n}{3}}=n^{1/3}.$ Therefore, $$\Pr_{\s}\left[ v_{i\ell}(\s)\geq \frac{\ln n}{3\ln\ln n}+1\right]\geq \frac{1}{en^{1/3}}.$$
	Let $X_{\ell}$ be the indicator for the event that item $\ell$ has value greater than $\frac{\ln n}{3\ln\ln n}$, and $X$ the number of such items in a set of $n$ items. We know that $$\mu=\E_{\s}\left[X\right] \geq n\cdot \frac{1}{en^{1/3}}=n^{2/3}/e.$$
	By Chebychev inequality, we have that 
	\begin{flalign*}
	\Pr_\s\left[\max_{\ell\in [n]}X_\ell \leq \frac{\ln n}{3\ln\ln n}+1\right] & \leq  \Pr_{\s}\left[\lvert X-\mu\rvert\geq \mu\right] \\
	&\leq  \frac{\Var(X)}{\mu^2}\\
	& \leq  e^2\cdot \frac{\sum_{\ell=1}^n(\Var(X_\ell))+\sum_{\ell\neq j}\Cov(X_\ell,X_j)}{n^{4/3}}. 
	\end{flalign*}
	%\ori{changed the first equality to inequality(it is not equal), in the last inequality the  denominator should be $n^{4/3}$ by my calculations}
	For each $\ell$, $\Var(X_\ell)\leq \E[X_\ell]^2= \frac{1}{e^2n^{2/3}},$ and since $X_\ell$ and $X_j$ are independent for each $\ell\neq j$, we also have that $\Cov(X_\ell,X_j)=0$ for each $\ell\neq j$. Therefore, we get $\Pr_\s\left[\max_{\ell\in [n]}X_\ell \leq \frac{\ln n}{3\ln\ln n}+1\right] \leq 1/n,$ %\ori{with the above change this should be $n^{-1}$} 
	which implies that $\E_\s[\max_{\ell\in [n]}v_{i\ell}(\s)]=\Omega(\ln n/\ln\ln n)$. This concludes the proof of the claim.	
\end{proof}	

The following claim is used to bound the expected value of the maximal item, and thus the number of items an agent bids on.
\begin{claim} \label{clm:expected-max-ub}
	For any $i$, and for any realization of $s_i=(s_{i1},\ldots,s_{im})$,
	$$\E_{\s_{-i}}\left[\max_\ell v_{i\ell}(\s)\ \Big\vert\ s_i\right]\leq 4\ln n/\ln\ln n+3.$$
\end{claim}


\begin{proof}
	Consider a bidder $i$. We have that 
	\begin{eqnarray}
	\Pr_{\s_{-i}}\left[\max_\ell v_{i\ell}(\s)\geq k+2\ \Big\vert\ s_i\right] & = & \Pr_{\s_{-i}}\left[\max_\ell\{ 1+\sum_{j\in[n]}s_{j\ell}\}\geq k+2\ \Big\vert\ s_i\right]\nonumber\\
	&\leq & \Pr_{\s_{-i}}\left[\max_\ell\{\sum_{j\neq i}s_{j\ell}\}\geq k\right]\nonumber\\
	& = & \Pr_{\s_{-i}}\left[\exists \ell\ :\ \sum_{j\neq i}s_{j\ell}\geq k\right]\nonumber\\
	&\leq & \Pr_{\s}\left[\exists \ell\ :\ \sum_{j\in [n]}s_{j\ell}\geq k\right]\nonumber\\
	&\leq & n^2\cdot \Pr_{\s}\left[ \sum_{j\in [n]}s_{j\ell}\geq k\right].\label{eq:highmax-bound}
	\end{eqnarray}
	The first inequality follows because the signals are sampled independently, and the best case is where $s_i$ is the all ones vector, and the last inequality is by applying a union bound. We can use a balls and bins type analysis in order to bound $\Pr_{\s}\left[ \sum_{j\in [n]}s_{j\ell}\geq k\right]$. Namely, If we consider any $k$ agents, the probability that these $k$ agents have a high signal for item $\ell$ is $\left(\frac{1}{n}\right)^k$. Using a union bound, we get that the probability there exist $k$ agents with a high signal for item $\ell$ is at most $\binom{n}{k}\left(\frac{1}{n}\right)^k$. Therefore, 
	\begin{eqnarray*}
		\Pr_{\s}\left[ \sum_{j\in [n]}s_{j\ell}\geq k\right] &\leq& \binom{n}{k}\left(\frac{1}{n}\right)^k\\
		&\leq& \left(\frac{en}{k}\right)^k\left(\frac{1}{n}\right)^k\\
		& = & \left(\frac{e}{k}\right)^k,
	\end{eqnarray*}
	where the second inequality follows Stirling's approximation. Setting $k=4\ln n/\ln\ln n$, we have that 
	\begin{eqnarray*}
		\Pr_{\s}\left[ \sum_{j\in [n]}s_{j\ell}\geq k\right] &\leq& \left(\frac{e\ln\ln n}{4\ln n}\right)^\frac{4\ln n}{\ln\ln n}\\
		& \leq & \exp\left(\frac{4\ln n}{\ln\ln n}(\ln\ln\ln n-\ln\ln n)\right)\\
		& = & \exp\left(-4\ln n + \frac{4\ln n\ln\ln\ln n}{\ln\ln n}\right),
	\end{eqnarray*}
	and for $n$ large enough,
	$$\Pr_{\s}\left[ \sum_{j\in [n]}s_{j\ell}\geq k\right] \leq \exp\left(-3\ln n\right) = \frac{1}{n^3}.$$
	Therefore, by Equation~\eqref{eq:highmax-bound},
	\begin{eqnarray}
	\Pr_{\s_{-i}}\left[\max_\ell v_{i\ell}(\s)\geq \frac{4\ln n}{\ln\ln n}+2\ \Big\vert\ s_i\right]\leq 1/n.
	\end{eqnarray}
	
	We get that 
	\begin{eqnarray*}
		\E_{\s_{-i}}\left[\max_\ell v_{i\ell}(\s)\ \Big\vert\ s_i\right]& \leq& \Pr_{\s_{-i}}\left[\max_\ell v_{i\ell}(\s)< \frac{4\ln n}{\ln\ln n}+2\ \Big\vert\ s_i\right]\cdot \left(\frac{4\ln n}{\ln\ln n}+2\right) \\
		& & \ +\ \Pr_{\s_{-i}}\left[\max_\ell v_{i\ell}(\s)\geq \frac{4\ln n}{\ln\ln n}+2\ \Big\vert\ s_i\right]\cdot (n+1) \\ 
		&\leq & (1-1/n)\cdot \left(\frac{4\ln n}{\ln\ln n}+2\right) + (n+1)/n\\
		& \leq & \frac{4\ln n}{\ln\ln n}+3.
	\end{eqnarray*}
	
\end{proof}

We also bound the expected value an agent might derive by bidding on a set of $\ln ^2n$ items. 
\begin{claim}\label{clm:expected-max-log2n-ub}
	If agent $i$ bids on a set of at most $\ln ^2n$ items, her expected value for that set is at most $\frac{4\ln\ln n }{\ln\ln\ln n}+4$ for any realization of $s_i$.
\end{claim}


\begin{proof}
	We first bound the probability that the agent sees an item with value greater than $\frac{4\ln\ln n }{\ln\ln\ln n}+2$. Notice that an agent chooses a set of items to bid on without knowing anything about the realization of the signals of other bidders. That is, if $S_i$ is that set of items $i$ bids on,
	\begin{eqnarray*}
		\Pr_{\s_{-i}}\left[\max_{\ell\in S_i} v_{i\ell}(\s) \geq k+2 \Big| s_i\right] &\leq& \Pr_{\s_{-i}}\left[\max_{\ell\in S_i} \sum_{j\neq i}s_{j\ell} \geq k\right]\\
		&\leq & |S_i|\Pr_{\s}\left[\sum_j s_{j\ell}\geq k\right]\\
		& \leq & \ln^2n\cdot\Pr_{\s}\left[\sum_j s_{j\ell}\geq k\right],
	\end{eqnarray*}
	where the derivations are similar to the ones in Claim~\ref{clm:expected-max-ub}.
	
	Using $k=\frac{4\ln\ln n }{\ln\ln\ln n},$ a similar progression to the one in Claim~\ref{clm:expected-max-ub} shows that 
	$$\Pr_{\s}\left[\sum_j s_{j\ell}\geq \frac{4\ln\ln n }{\ln\ln\ln n}\right] \leq \ln^{-3} n,$$
	which yields $$\Pr_{\s_{-i}}\left[\max_{\ell\in S_i} v_{i\ell}(\s) \geq \frac{4\ln\ln n }{\ln\ln\ln n}+2 \Big| s_i\right] \leq \frac{1}{\ln n}.$$
	
	We conclude by noting that 
	\begin{eqnarray*}
		\E_{\s_{-i}}\left[\max_{\ell\in S_i} v_{i\ell}(\s) \right] &\leq& \Pr_{\s_{-i}} \left[\max_{\ell\in S_i} v_{i\ell}(\s) \leq \frac{4\ln\ln n }{\ln\ln\ln n}+2 \Big| s_i\right]\cdot  \left(\frac{4\ln\ln n }{\ln\ln\ln n}+2\right) \\
		& & + \Pr_{\s_{-i}} \left[\frac{4\ln\ln n }{\ln\ln\ln n}+2 \leq \max_{\ell\in S_i} v_{i\ell}(\s) \leq \frac{4\ln n }{\ln\ln n}+2 \Big| s_i\right]\cdot  \left(\frac{4\ln n }{\ln\ln n}+2\right)\\
		& & + \Pr_{\s_{-i}}\left[\max_{\ell\in S_i} v_{i\ell}(\s)\geq \frac{4\ln n }{\ln\ln n}+2 \Big| s_i\right]\cdot  \left(n+1\right)\\
		&\leq & \left(\frac{4\ln\ln n }{\ln\ln\ln n}+2\right) + \frac{1}{\ln n}\left(\frac{4\ln n }{\ln\ln n}+2\right) + \frac{1}{n}(n+1)\\
		&\leq & \frac{4\ln\ln n }{\ln\ln\ln n} +2 +4/\ln\ln n+2/\ln n + 1 + 1/n\\
		&\leq& \frac{4\ln\ln n }{\ln\ln\ln n}+4,
	\end{eqnarray*} 
	which completes the proof.
\end{proof}


With these claims in hand, we are ready to establish the proof of Theorem~\ref{thm:multi-neg}.

\begin{proof}[Proof (of Theorem~\ref{thm:multi-neg})]
	Let $S_i$ be the random set of items agent $i$ bids on. We can bound the expected size of $S_i$ for every $s_i$ by
	\begin{eqnarray}
	\E[\lvert S_i\rvert \mid s_i]\ \leq\ \E_{\substack{\s_{-i}\sim\F_{-i}\\(b_i,a_i)\sim \sigma_i(s_i)}}\left[\sum_{\ell\ :\ a_{i\ell}=1}v_{i\ell}(b_{i\ell},\s_{-i})\right]\ \leq\ \E_{\s_{-i}\sim\F_{-i}}\left[v_{i}(S_i;\s)\right]\ \leq\ \frac{4\ln n}{\ln\ln n}+3.\label{eq:bid-set-ub}
	\end{eqnarray}
	The first inequality in \eqref{eq:bid-set-ub} follows by the fact that the value is at least 1 for every item and agent, the second inequality follows by no-overbidding, and the third inequality follows by Claim~\ref{clm:expected-max-ub}.
	
	By Markov inequality, and by Equation~\eqref{eq:bid-set-ub}, we have that for every $s_i$, 
	\begin{eqnarray*}
		\Pr\left[\lvert S_i\rvert> \ln^2n \mid s_i\right] < \frac{\frac{4\ln n}{\ln\ln n}+3}{\ln^2n}=O(1/\ln n\ln\ln n).
	\end{eqnarray*}
	\vspace{-3pt}
	We now get that for every $s_i$
	\vspace{-3pt}
	\begin{eqnarray*}
		\E_{\s_{-i}, S_i}\left[v_i(S_i;\s) \mid s_i\right]&\leq& \Pr\left[|S_i| \leq \ln^2 n \mid s_i\right]\left(\frac{4\ln\ln n }{\ln\ln\ln n}+4\right)\ +\ \Pr\left[|S_i| > \ln^2 n \mid s_i\right]\cdot \left(\frac{4\ln n}{\ln\ln n}+3\right)\\
		& = & O\left(\frac{\ln\ln n}{\ln\ln\ln n}\right)+ O\left(\frac{1}{\ln n\ln\ln n}\frac{\ln n}{\ln\ln n}\right) \ = \  O\left(\frac{\ln\ln n}{\ln\ln\ln n}\right),
	\end{eqnarray*}
	where the first inequality follows by Claims~\ref{clm:expected-max-ub} and~\ref{clm:expected-max-log2n-ub}.
	
	Therefore, the expected value of the set of items an agent $i$ bids on is $\E_{\s, S_i}\left[v_i(S_i;\s)\right]= O\left(\frac{\ln\ln n}{\ln\ln\ln n}\right)$. Since this is an upper bound on the value of items the agent wins, every agent gets a value of $O\left(\frac{\ln\ln n}{\ln\ln\ln n}\right)$ in an equilibrium, thus $\eq(\sigma)= O(n\ln\ln n/\ln\ln\ln n)$. Since $\opt= \Omega\left(n\ln n/\ln\ln n\right)$ (by Claim~\ref{clm:opt-lb}), we conclude that $\opt/\eq = \Omega(\ln n\ln\ln\ln n/\ln\ln^2 n)$.
	
	This concludes the proof Theorem~\ref{thm:multi-neg}.
\end{proof}



==> multiple-neg.tex <==
In this section, we show that for the case of multiple items, there is a dichotomy between the case of few and many items; namely, one cannot hope for a bound independent of $n$, even in the very simple case of (a) \textit{Common values} (which implies $\gamma=c=1$); (b) \textit{Symmetric valuations:} the valuation functions describing each of the items are identical, and each agent/item signal is drawn i.i.d.\footnote{Moreover, the valuations satisfy the diminishing marginal influence Definitions~\ref{cond:strong_submod} and~\ref{cond:weak_submod}.}; (c) $\widetilde{\opt}/\opt\longrightarrow 1$ as $n$ grows large.

\begin{restatable}{theorem}{mainneg}
	\label{thm:multi-neg}
	There exists an instance with $n$ unit-demand agents and $n^2$ items, with $\gamma=c=1$, and $\widetilde{\opt}\approx\opt$, where under a no-overbidding assumption, for every item-bidding mechanism and every equilibrium $\sigma$,
	$\opt/\eq(\sigma)=\Omega(\ln n\ln\ln\ln n/\ln\ln^2 n)$.
\end{restatable}

\begin{proof}[Proof (Sketch)]

In our setting, each agent $i$ has a signal $s_{i\ell}$ for each item $\ell$, which is distributed according to $$s_{i\ell}=\begin{cases}
1\quad \text{w.p. } 1/n\\
0\quad \text{w.p. } 1-1/n
\end{cases},$$ independently (and identically) of other items. There are $n^2$ items, and the valuation function for each agent $i$ and item $\ell$ is $v_{i\ell}(\s)=1+\sum_j s_{j\ell}.$ 

In Theorem \ref{thm:multi-neg} we establish a gap between the optimal welfare and the welfare in equilibrium that is a function of $n$. Before presenting the result, we provide a high-level description of it along with some intuition.
\begin{itemize}
	\item Consider an arbitrary set of $n$ items. There are roughly $n$ high signals distributed on items in this set roughly uniformly. One can use a balls-and-bins type analysis to show that the highest-valued item in this set has value roughly $\ln n/\ln\ln n,$ up to constant factors (See Claim~\ref{clm:opt-lb}). Therefore, if one partitions the $n^2$ items arbitrarily into $n$ sets of size~$n$, and assigns the highest-valued item in each set to a different agent (this assignment can be arbitrary, due to common value), the obtained welfare is roughly $n\ln n/\ln\ln n.$
	\item Next, we bound the number of items an agent bids on by applying a no-overbidding assumption. Assume an agent bids on a set of items of size~$k$. Since the value of each item is at least~1, the sum of the agent's bids is at least~$k$. On the other hand, the value of any set of items is upper bounded by the value of the grand bundle, which is roughly~$\ln n/\ln\ln n$ (this is roughly the value of the highest-valued item in the grand bundle, according to a balls-and-bins type analysis) (see Claim~\ref{clm:expected-max-ub}). Therefore, the no-overbidding assumption implies that the expected number of items an agent bids on is $O(\ln n/\ln\ln n)$ (See Equation~\eqref{eq:bid-set-ub}).
	\item Finally, since an agent has a very vague idea about the valuable items (she only knows the $+1$ her signal may contribute to some of the items), the agent's bid is basically `a shot in the dark'. Using a balls-and-bins type analysis again, we show that the expected value an agent derives from the items she bids on is $O(\ln\ln n /\ln\ln\ln n)$ (see Claim~\ref{clm:expected-max-log2n-ub}), implying that $\eq = O(n\ln\ln n /\ln\ln\ln n)$, which yields a lower bound of $\tilde{\Omega}(\ln n).$\footnote{Here, $\tilde{\Omega}$ hides away terms that are $o(\ln n)$.}
\end{itemize} 
\end{proof}
The formal proof appears in Appendix~\ref{appx:multiple-neg}

%\ori{if using $\tilde{\Omega}$ then we should probably explain this notation, otherwise we can copy the full expression from below}


%\alon{Rephrased the statement again, please review.}




